Delay Analysis of IEEE 802.11be Multi-link Operation under Finite Load

Multi-link Operation (MLO), arguably the most disruptive feature introduced in IEEE 802.11be, will cater for delay-sensitive applications by using multiple radio interfaces concurrently. In this paper, we analyze the delay distribution of MLO under non-saturated traffic. Our results show that upgrading from legacy single-link to MLO successfully contains the $95$th percentile delay as the traffic load increases, but also that adding extra interfaces yields rapidly diminishing gains. Further experiments we conduct on Google Stadia traces, accounting for realistic traffic with batch arrivals, confirm the insights stemming from our theoretical analysis, vouching for MLO to support high-resolution real-time video with a controlled delay.

==> 0X_Algorithm.tex <==
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\begin{algorithm}
\caption{Numerical computation of the delay distribution}\label{alg:cap}
\begin{algorithmic}[1]
\Require Channel occupancy $\rho$, collision probability $p$, packet arrival rate $\lambda$, number of interfaces $S$. 
\Ensure Delay distribution $F_D(t)$.\\
Initialize $\E[B] = \mathrm{CW}/2$ and $\pi_0 = 1$.\\
Set $\rho$ and $p$ from data or compute them from (\ref{Eq:rho}) and (\ref{Eq:p}).
\While{Convergence has not been reached}
\State Calculate $\E[D_{\mathrm{s}}]$ from $\E[B]$, $p$, and $\rho$ using (\ref{Eq:service_time}).
\State Calculate $a$ and $\mu$ from $\E[D_{\mathrm{s}}]$ using (\ref{Eq:mu_a}).
\State Calculate $\pi_n$ from $a$ using (\ref{eqn:pi_n}) and (\ref{eqn:pi_0}).
\State Calculate $\E[B]$ from $\pi_n$ using (\ref{Eq:MeanBackoffOverN}).
\EndWhile
\State Calculate $F_D(t)$ from $a$ and $\mu$ using (\ref{Eq:CDF}) and (\ref{Eq:eta}).
\end{algorithmic}
\label{Algo}
\end{algorithm}

==> 0X_Algorithm1.tex <==
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\begin{algorithm}
\caption{Numerical computation of the delay distribution}\label{alg:cap}
\begin{algorithmic}[1]
\Require Packet arrival rate $\lambda$, number of interfaces $S$, number of contenders per interface $N_c$ 
\Ensure Delay distribution $F_D(t)$.\\
Initialize $\E[B] = \mathrm{CW}/2$ and $\pi_0 = 1$.\\
%Set $\rho$ and $p$ from data or compute them from (\ref{Eq:rho}) and (\ref{Eq:p}).
\While{Convergence has not been reached}
\State Calculate $\tau$, $p'$, $\tau_m$, $p$, $\E[B']$ and $\rho$.
%
\While{Convergence has not been reached}
\State Calculate $\E[D_{\mathrm{s}}]$ from $\E[B_m]$, $p$, and $\rho$ using (\ref{Eq:service_time}).
%
\State Calculate $a$ and $\mu$ from $\E[D_{\mathrm{s}}]$ using (\ref{Eq:mu_a}).
%
\State Calculate $\pi_n$ from $a$ using (\ref{eqn:pi_n}) and (\ref{eqn:pi_0}).
%
\State Calculate $\E[B]$ from $\pi_n$ using (\ref{Eq:MeanBackoffOverN}).
\EndWhile
\EndWhile
%
\State Calculate $F_D(t)$ from $a$ and $\mu$ using (\ref{Eq:CDF}) and (\ref{Eq:eta}).
\end{algorithmic}
\label{Algo}
\end{algorithm}
